Finite temperature geometric properties of the Kitaev honeycomb model

We study finite temperature topological phase transitions of the Kitaev's spin honeycomb model in the vortex-free sector with the use of the recently introduced mean Uhlmann curvature. We employ an appropriate Fermionisation procedure to study the system as a two-band p-wave superconductor described by a BdG Hamiltonian. This allows to study relevant quantities such as Berry and mean Uhlmann curvatures in a simple setting. More specifically, we consider the spin honeycomb in the presence of an external magnetic field breaking time reversal symmetry. The introduction of such an external perturbation opens a gap in the phase of the system characterised by non-Abelian statistics, and makes the model to belong to a symmetry protected class, so that the Uhmann number can be analysed. We first consider the Berry curvature on a particular evolution line over the phase diagram. The mean Uhlmann curvature and the Uhlmann number are then analysed considering the system to be in a Gibbs state at finite temperature. Then, we show that the mean Uhlmann curvature describes a cross-over effect of the phases at high temperature. We also find an interesting nonmonotonic behaviour of the Uhlmann number as a function of the temperature in the trivial phase, which is due to the partial filling of the conduction band around Dirac points.

==> ref.bib-save-2019.02.11.16.41.40 <==


@article{Altland1997,
  author =        {Altland, Alexander and Zirnbauer, Martin R},
  journal =       {Phys. Rev. B},
  month =         {jan},
  number =        {2},
  pages =         {1142--1161},
  title =         {{Nonstandard symmetry classes in mesoscopic
                   normal-superconducting hybrid structures}},
  volume =        {55},
  year =          {1997},
  doi =           {10.1103/PhysRevB.55.1142},
  issn =          {0163-1829},
  url =           {https://link.aps.org/doi/10.1103/PhysRevB.55.1142},
}

@article{Schnyder2008,
  author =        {Schnyder, Andreas P. and Ryu, Shinsei and
                   Furusaki, Akira and Ludwig, Andreas W. W.},
  journal =       {Phys. Rev. B},
  month =         {nov},
  number =        {19},
  pages =         {195125},
  title =         {{Classification of topological insulators and
                   superconductors in three spatial dimensions}},
  volume =        {78},
  year =          {2008},
  abstract =      {We systematically study topological phases of
                   insulators and superconductors (SCs) in 3D. We find
                   that there exist 3D topologically non-trivial
                   insulators or SCs in 5 out of 10 symmetry classes
                   introduced by Altland and Zirnbauer within the
                   context of random matrix theory. One of these is the
                   recently introduced Z{\_}2 topological insulator in
                   the symplectic symmetry class. We show there exist
                   precisely 4 more topological insulators. For these
                   systems, all of which are time-reversal (TR)
                   invariant in 3D, the space of insulating ground
                   states satisfying certain discrete symmetry
                   properties is partitioned into topological sectors
                   that are separated by quantum phase transitions. 3 of
                   the above 5 topologically non-trivial phases can be
                   realized as TR invariant SCs, and in these the
                   different topological sectors are characterized by an
                   integer winding number defined in momentum space.
                   When such 3D topological insulators are terminated by
                   a 2D surface, they support a number (which may be an
                   arbitrary non-vanishing even number for singlet
                   pairing) of Dirac fermion (Majorana fermion when spin
                   rotation symmetry is completely broken) surface modes
                   which remain gapless under arbitrary perturbations
                   that preserve the characteristic discrete symmetries.
                   In particular, these surface modes completely evade
                   Anderson localization. These topological phases can
                   be thought of as 3D analogues of well known paired
                   topological phases in 2D such as the chiral p-wave
                   SC. In the corresponding topologically non-trivial
                   and topologically trivial 3D phases, the
                   wavefunctions exhibit markedly distinct behavior.
                   When an electromagnetic U(1) gauge field and
                   fluctuations of the gap functions are included in the
                   dynamics, the SC phases with non-vanishing winding
                   number possess non-trivial topological ground state
                   degeneracies.},
  doi =           {10.1103/PhysRevB.78.195125},
  isbn =          {9780735406711},
  issn =          {1098-0121},
  url =           {https://link.aps.org/doi/10.1103/PhysRevB.78.195125},
}

@article{Ryu2010,
  author =        {Ryu, Shinsei and Schnyder, Andreas P. and
                   Furusaki, Akira and Ludwig, Andreas W W},
  journal =       {New J. Phys.},
  month =         {jun},
  number =        {6},
  pages =         {065010},
  title =         {{Topological insulators and superconductors: tenfold
                   way and dimensional hierarchy}},
  volume =        {12},
  year =          {2010},
  abstract =      {It has recently been shown that in every spatial
                   dimension there exist precisely five distinct classes
                   of topological insulators or superconductors. Within
                   a given class, the different topological sectors can
                   be distinguished, depending on the case, by a Z or a
                   Z 2 topological invariant. This is an exhaustive
                   classification. Here we construct representatives of
                   topological insulators and superconductors for all
                   five classes and in arbitrary spatial dimension d, in
                   terms of Dirac Hamiltonians. Using these
                   representatives we demonstrate how topological
                   insulators (superconductors) in different dimensions
                   and different classes can be related via 'dimensional
                   reduction' by compactifying one or more spatial
                   dimensions (in 'Kaluza–Klein'-like fashion). For
                   Z-topological insulators (superconductors) this
                   proceeds by descending by one dimension at a time
                   into a different class. The Z 2 -topological
                   insulators (superconductors), on the other hand, are
                   shown to be lower-dimensional descendants of parent
                   Z-topological insulators in the same class, from
                   which they inherit their topological properties. The
                   eightfold periodicity in dimension d that exists for
                   topological insulators (superconductors) with
                   Hamiltonians satisfying at least one reality
                   condition (arising from time-reversal or
                   charge-conjugation/particle–hole symmetries) 2 is a
                   reflection of the eightfold periodicity of the spinor
                   representations of the orthogonal groups SO(N) (a
                   form of Bott periodicity). Furthermore, we derive for
                   general spatial dimensions a relation between the
                   topological invariant that characterizes topological
                   insulators and superconductors with chiral symmetry
                   (i.e., the winding number) and the Chern–Simons
                   invariant. For lower-dimensional cases, this formula
                   relates the winding number to the electric
                   polarization (d = 1 spatial dimensions) or to the
                   magnetoelectric polarizability (d = 3 spatial
                   dimensions). Finally, we also discuss topological
                   field theories describing the spacetime theory of
                   linear responses in topological insulators
                   (superconductors) and study how the presence of
                   inversion symmetry modifies the classification of
                   topological insulators (superconductors).},
  doi =           {10.1088/1367-2630/12/6/065010},
  isbn =          {1367-2630},
  issn =          {1367-2630},
  url =           {http://stacks.iop.org/1367-2630/12/i=6/a=065010?
                  key=crossref.8100f885f6d94a261914942850e92d50},
}

@article{Chiu2016,
  author =        {Chiu, Ching-Kai and Teo, Jeffrey C. Y. and
                   Schnyder, Andreas P. and Ryu, Shinsei},
  journal =       {Rev. Mod. Phys.},
  month =         {aug},
  number =        {3},
  pages =         {035005},
  title =         {{Classification of topological quantum matter with
                   symmetries}},
  volume =        {88},
  year =          {2016},
  abstract =      {Topological materials have become the focus of
                   intense research in recent years, since they exhibit
                   fundamentally new physical phenomena with potential
                   applications for novel devices and quantum
                   information technology. One of the hallmarks of
                   topological materials is the existence of protected
                   gapless surface states, which arise due to a
                   nontrivial topology of the bulk wave functions. This
                   review provides a pedagogical introduction into the
                   field of topological quantum matter with an emphasis
                   on classification schemes. We consider both fully
                   gapped and gapless topological materials and their
                   classification in terms of global symmetries, such as
                   time-reversal, as well as spatial symmetries, such as
                   reflection. Furthermore, we survey the classification
                   of gapless modes localized on topological defects.
                   The classification of these systems is discussed by
                   use of homotopy groups, Clifford algebras, K-theory,
                   and non-linear sigma models describing the Anderson
                   (de-)localization at the surface or inside a defect
                   of the material. Theoretical model systems and their
                   topological invariants are reviewed together with
                   recent experimental results in order to provide a
                   unified and comprehensive perspective of the field.
                   While the bulk of this article is concerned with the
                   topological properties of noninteracting or
                   mean-field Hamiltonians, we also provide a brief
                   overview of recent results and open questions
                   concerning the topological classifications of
                   interacting systems.},
  doi =           {10.1103/RevModPhys.88.035005},
  isbn =          {9781479957514},
  issn =          {0034-6861},
  url =           {https://link.aps.org/doi/10.1103/RevModPhys.88.035005},
}

@article{Hatsugai1993,
  author =        {Hatsugai, Yasuhiro},
  journal =       {Phys. Rev. Lett.},
  month =         {nov},
  number =        {22},
  pages =         {3697--3700},
  title =         {{Chern number and edge states in the integer quantum
                   Hall effect}},
  volume =        {71},
  year =          {1993},
  doi =           {10.1103/PhysRevLett.71.3697},
  issn =          {0031-9007},
  url =           {https://link.aps.org/doi/10.1103/PhysRevLett.71.3697},
}

@article{Klitzing1980,
  author =        {Klitzing, K V and Dorda, G and Pepper, M},
  journal =       {Phys. Rev. Lett.},
  month =         {aug},
  number =        {6},
  pages =         {494--497},
  title =         {{New Method for High-Accuracy Determination of the
                   Fine-Structure Constant Based on Quantized Hall
                   Resistance}},
  volume =        {45},
  year =          {1980},
  abstract =      {Measurements of the Hall voltage of a two-di ' 1 I
                   {\~{}} ] 0 {\~{}} {\~{}} wo-imensiona electron gas,
                   realized with a si icon metal-oxide-semiconductor
                   field-effect transistor, show that the Hall resi at
                   particular, experimentall well-d ow a e a resistance
                   which de end onl y we -e ined surface carrier
                   concentrations h f' d p y on the fine-structure
                   constant and speed of li ht d ' as ixe va ues the
                   come tr g ry of the device. Preliminary data are
                   reported. {\~{}} {\~{}} {\~{}} o ig, an is
                   insensitive to PACS numbers: 73.25.+i, 06.20.Jr,
                   72.20.My, 73.40.Qv In this paper we report a new,
                   potentially high-accuracy method for determining the
                   fine-struc-ture constant, n. The new approach is
                   based on the fact that the degenerate electron gas in
                   the in-version layer of a MOSFET
                   (metal-oxide-semi-conductor field-effect transistor)
                   is fully cluan-tized when the transistor is operated
                   at helium temperatures and in a strong magnetic field
                   of order 15 T. ' The inset in Fig. 1 shows a
                   schem-atic diagram of a typical MOSFET device used in
                   this work. The electric field perpendicular to the
                   surface (gate field) produces subbands for the
                   mo-tion normal to the semiconductor-oxide interface,
                   and the magnetic field produces Landau quantiza-tion
                   of motion parallel to the interface. The den-sity of
                   states D(E) consists of broadened 5 func-tions';
                   minimal overlap is achieved if the mag-netic field is
                   sufficiently high.},
  doi =           {10.1103/PhysRevLett.45.494},
  isbn =          {0031-9007},
  issn =          {0031-9007},
  url =           {https://journals.aps.org/prl/pdf/10.1103/
                  PhysRevLett.45.494 https://link.aps.org/doi/10.1103/
                  PhysRevLett.45.494},
}

@article{Thouless1982,
  author =        {Thouless, D. J. and Kohmoto, M. and
                   Nightingale, M. P. and den Nijs, M.},
  journal =       {Phys. Rev. Lett.},
  month =         {aug},
  number =        {6},
  pages =         {405--408},
  title =         {{Quantized Hall Conductance in a Two-Dimensional
                   Periodic Potential}},
  volume =        {49},
  year =          {1982},
  abstract =      {The Hall conductance of a two-dimensional electron
                   gas has been studied in a uniform magnetic field and
                   a periodic substrate potential U. The Kubo formula is
                   written in a form that makes apparent the
                   quantization when the Fermi energy lies in a gap.
                   Explicit expressions have been obtained for the Hall
                   conductance for both large and small U/$\omega$c.},
  doi =           {10.1103/PhysRevLett.49.405},
  isbn =          {0031-9007},
  issn =          {0031-9007},
  url =           {https://link.aps.org/doi/10.1103/PhysRevLett.49.405},
}

@article{Thouless1983,
  author =        {Thouless, D. J.},
  journal =       {Phys. Rev. B},
  number =        {10},
  pages =         {6083--6087},
  title =         {{Quantization of particle transport}},
  volume =        {27},
  year =          {1983},
  abstract =      {The integrated particle current produced by a slow
                   periodic variation of the potential of a Schrodinger
                   equation is evaluated. It is shown that in a finite
                   torus the integral of the current over a period can
                   vary continuously, but in an infinite periodic system
                   with full bands it must have an integer value. This
                   quantization of particle transport is used to clas-
                   sify the energy gaps in a one-dimensional system with
                   competing or incommensurate periods. It is also used
                   to rederive Prange's results for the fractional
                   charge of a soliton.},
  doi =           {10.1103/PhysRevB.27.6083},
  issn =          {01631829},
}

@article{Niu1984,
  author =        {Niu, Q. and Thouless, D. J.},
  journal =       {J. Phys. A Gen. Phys.},
  number =        {12},
  pages =         {2453--2462},
  title =         {{Quantised adiabatic charge transport in the presence
                   of substrate disorder and many-body interaction}},
  volume =        {17},
  year =          {1984},
  abstract =      {The result for the quantised charge transport induced
                   by an adiabatically varying substrate potential is
                   generalised to the case in which both substrate
                   disorder and many-body interaction are present. The
                   application of our theory to the problem of the
                   integral and fractional quantised Hall effect is
                   discussed.},
  doi =           {10.1088/0305-4470/17/12/016},
  isbn =          {10.1088/0305-4470/17/12/016},
  issn =          {03054470},
}

@article{Nakajima2016,
  author =        {Nakajima, Shuta and Tomita, Takafumi and
                   Taie, Shintaro and Ichinose, Tomohiro and
                   Ozawa, Hideki and Wang, Lei and Troyer, Matthias and
                   Takahashi, Yoshiro},
  journal =       {Nat. Phys.},
  month =         {apr},
  number =        {4},
  pages =         {296--300},
  title =         {{Topological Thouless pumping of ultracold fermions}},
  volume =        {12},
  year =          {2016},
  abstract =      {A gas of electrons in a one-dimensional periodic
                   potential can be transported even in the absence of a
                   voltage bias if the potential is modulated slowly and
                   periodically in time. Remarkably, the transferred
                   charge per cycle is only sensitive to the topology of
                   the path in parameter space. Although this so-called
                   Thouless charge pump has first been proposed more
                   than thirty years ago, it has not yet been realized.
                   Here we report the first demonstration of topological
                   Thouless pumping using ultracold atoms in a
                   dynamically controlled optical superlattice. We
                   observe a shift of the atomic cloud as a result of
                   pumping and extract the topological invariance of the
                   pumping process from this shift. We demonstrate the
                   topological nature of the Thouless pump by varying
                   the topology of the pumping path and verify that the
                   topological pump indeed works in the quantum region
                   by varying speed and temperature.},
  doi =           {10.1038/nphys3622},
  isbn =          {1745-2473},
  issn =          {1745-2473},
  url =           {http://www.nature.com/articles/nphys3622},
}

@article{Tsui1982,
  author =        {Tsui, D. C. and Stormer, H. L. and Gossard, A. C.},
  journal =       {Phys. Rev. Lett.},
  month =         {may},
  number =        {22},
  pages =         {1559--1562},
  title =         {{Two-Dimensional Magnetotransport in the Extreme
                   Quantum Limit}},
  volume =        {48},
  year =          {1982},
  abstract =      {A quantized Hall plateau of p» — — 31'/e,
                   accompanied by a minimum in p " , was observed at
                   {\&} {\&} 5 K in magnetotransport of high-mobility,
                   bvo-dimensional electrons, when the low-est-energy,
                   spin-polarized Landau level is 3 filled. The
                   formation of a Wigner solid or charge-density-wave
                   state with triangular symmetry is suggested as a
                   possible explana-tion. PACS numbers: 72.20. My,
                   71.45.-d, 73.40.Lq, 73.60.Fw In the presence of an
                   intense perpendicular magnetic field B, a system of
                   two-dimensional (2D) electrons is expected to form a
                   Wigner sol-id' at low temperatures (T). In the
                   infinite-B limit, an analogy can be drawn to the
                   classical electron gas on the surface of liquid
                   helium, which crystallizes into a solid' when the
                   ratio of the electron's average potential energy to
                   therma1. energy I'=-e'm'{\~{}}'n/ekT=137 (n is the
                   electron areal density). At finite B, quantum effects
                   be-come important and it has been suggested that a
                   charge-density-wave (CDW) state' may be pos-sible at
                   considerabl. y higher T as a precursor to Wigner
                   crystallization. Early experiments were carried out
                   on the Si inversion layer at the Si-SiO, interface.
                   Kawaji and Wakabayashi' and Tsui' made high-B
                   magnetoconductivity measure-ments and observed
                   structures and electric field dependences which
                   cannot be explained by the in-dependent-electron
                   theory of Ando and Uemura. ' Subsequently, Kennedy et
                   al. ' observed a shift in cyclotron resonance,
                   concomitant with a drastic line narrowing, in the
                   high-B limit, when the average electron separation
                   exceeds the cyclo-tron diameter. Wilson, Allen, and
                   Tsui' studied the dependence of this phenomenon on
                   the Landau-level filling factor (v = nb/eB), and
                   found that a pinned-CDW model'o gave the most
                   satisfactory account of the cyclotron resonance data.
                   However, in the range of n at which these experiments
                   were performed, localization due to disorder at the
                   Si-SiO, interface is known to be important even in
                   the absence of B, and consequently, it has not been
                   possible to discern true Coulomb effects from those
                   due to disorder. In this Letter, we report some
                   striking, new results on the transport of
                   high-mobility, 2D electrons, in GaAs-AlGaAs
                   heterojunctions, in the extreme quantum limit (v {\&}
                   I), when the low-est-energy, spin-polarized Landau
                   level is par-tially filled. We found that at
                   temperatures T{\&} 5 K, the diagonal part p " " of
                   the resistivity tensor shows a dip at v = —, ',
                   which becomes stronger at lower T. For v {\&} —, ',
                   p " " follows an approximately exponential increase
                   with inverse T. The Hall resistivity p " " on the
                   other hand, approaches a step of Sh/e' at v = —, '
                   as T decreases, but re-mains essentially independent
                   of T away from this Hall plateau. These features of
                   the data re-semble those of the quantized Hall
                   resistance and the zero-resistance state expected
                   exclusively for integral values of v. We suggest that
                   these strik-ing results are evidence for a new
                   electronic state at v = —, '. They are consistent
                   with the no-tion that a Wigner solid, or a CDW state
                   with triangular crystal symmetry, is favored at v =
                   —, ' when the unit cell area of the lattice is a
                   multi-ple of the area of a magnetic flux quantum. The
                   samples, consisting of 1-p,m undoped GaAs, 500-A
                   undoped Al, , Ga, Ps, 600-A Si-doped Al, , Ga, gs,
                   and 200-A Si-doped GaAs single crystals were
                   sequentially grown on insulating GaAs substrates
                   using molecular-beam-epitaxy techniques. " The 2D
                   electron gas, resulting from ionized donors placed
                   500 A inside AlGaAs, " is established at the undoped
                   GaAs side of the GaAs-AlGaAs heterojunction. Samp1.
                   es were cut into standard Hall bridges and Ohmic
                   contacts to the electron layer were made with In at
                   400'C. Low-field transport measurements were used to
                   deter-mine n and p, . Our samples have n from 1.
                   1{\~{}}10" to 1.4{\&} 10" cm and p, from 80000 to
                   100000 cm'/V sec. The high-B measurements were
                   per-formed at the Francis Bitter National Magnet
                   Laboratory, Cambridge, Mass. Figure 1 shows p " , and
                   p " " of one specimen as a function of B at four
                   different temperatures. The scale at the top of the
                   figure shows the Lan-dau level filling factor v,
                   which gives the number of occupied levels. At
                   integral values of v, the data show the
                   characteristic features of the quan-tized Hall
                   plateaus and the vanishing of p " " , " " when the
                   Fermi energy EF is pinned in the gap between two
                   adjacent 1.evels. Removal of spin de-Qc 1982 The
                   American Physical Society 1559},
  doi =           {10.1103/PhysRevLett.48.1559},
  isbn =          {9788578110796},
  issn =          {0031-9007},
  url =           {https://link.aps.org/doi/10.1103/PhysRevLett.48.1559},
}

@article{Laughlin1983,
  author =        {Laughlin, R. B.},
  journal =       {Phys. Rev. Lett.},
  month =         {may},
  number =        {18},
  pages =         {1395--1398},
  title =         {{Anomalous Quantum Hall Effect: An Incompressible
                   Quantum Fluid with Fractionally Charged Excitations}},
  volume =        {50},
  year =          {1983},
  doi =           {10.1103/PhysRevLett.50.1395},
  issn =          {0031-9007},
  url =           {https://link.aps.org/doi/10.1103/PhysRevLett.50.1395},
}

@misc{Arovas1984,
  author =        {Arovas, Daniel P and Schrieffer, J R and Wilczek, F},
  booktitle =     {Phys. Rev. Lett.},
  number =        {7},
  pages =         {722--723},
  title =         {{Fraction statistics and the Quantum Hall effect}},
  volume =        {53},
  year =          {1984},
  doi =           {10.1103/PhysRevLett.53.722},
  issn =          {0031-9007},
  url =           {papers2://publication/uuid/E61AB9D9-FE7B-4EA4-9244-
                  1147363676D5},
}

@article{Nayak2008,
  author =        {Nayak, Chetan and Simon, Steven H. and Stern, Ady and
                   Freedman, Michael and {Das Sarma}, Sankar},
  journal =       {Rev. Mod. Phys.},
  month =         {sep},
  number =        {3},
  pages =         {1083--1159},
  title =         {{Non-Abelian anyons and topological quantum
                   computation}},
  volume =        {80},
  year =          {2008},
  abstract =      {Topological quantum computation has recently emerged
                   as one of the most exciting approaches to
                   constructing a fault-tolerant quantum computer. The
                   proposal relies on the existence of topological
                   states of matter whose quasiparticle excitations are
                   neither bosons nor fermions, but are particles known
                   as {\{}$\backslash$it Non-Abelian anyons{\}}, meaning
                   that they obey {\{}$\backslash$it non-Abelian
                   braiding statistics{\}}. Quantum information is
                   stored in states with multiple quasiparticles, which
                   have a topological degeneracy. The unitary gate
                   operations which are necessary for quantum
                   computation are carried out by braiding
                   quasiparticles, and then measuring the
                   multi-quasiparticle states. The fault-tolerance of a
                   topological quantum computer arises from the
                   non-local encoding of the states of the
                   quasiparticles, which makes them immune to errors
                   caused by local perturbations. To date, the only such
                   topological states thought to have been found in
                   nature are fractional quantum Hall states, most
                   prominently the $\backslash$nu=5/2 state, although
                   several other prospective candidates have been
                   proposed in systems as disparate as ultra-cold atoms
                   in optical lattices and thin film superconductors. In
                   this review article, we describe current research in
                   this field, focusing on the general theoretical
                   concepts of non-Abelian statistics as it relates to
                   topological quantum computation, on understanding
                   non-Abelian quantum Hall states, on proposed
                   experiments to detect non-Abelian anyons, and on
                   proposed architectures for a topological quantum
                   computer. We address both the mathematical
                   underpinnings of topological quantum computation and
                   the physics of the subject using the
                   $\backslash$nu=5/2 fractional quantum Hall state as
                   the archetype of a non-Abelian topological state
                   enabling fault-tolerant quantum computation.},
  doi =           {10.1103/RevModPhys.80.1083},
  isbn =          {0034-6861},
  issn =          {0034-6861},
  url =           {https://link.aps.org/doi/10.1103/RevModPhys.80.1083},
}

@article{Avron2011,
  author =        {Avron, J. E. and Fraas, M. and Graf, G. M. and
                   Kenneth, O.},
  journal =       {New J. Phys.},
  month =         {may},
  number =        {5},
  pages =         {053042},
  title =         {{Quantum response of dephasing open systems}},
  volume =        {13},
  year =          {2011},
  abstract =      {We develop a theory of adiabatic response for open
                   systems governed by Lindblad evolutions. The theory
                   determines the dependence of the response
                   coefficients on the dephasing rates and allows for
                   residual dissipation even when the ground state is
                   protected by a spectral gap. We give the quantum
                   response a geometric interpretation in terms of
                   Hilbert space projections: for a two-level system
                   and, more generally, for systems with a suitable
                   functional form of the dephasing, the dissipative and
                   non-dissipative parts of the response are linked to a
                   metric and to a symplectic form. The metric is the
                   Fubini–Study metric and the symplectic form is the
                   adiabatic curvature. When the metric and symplectic
                   structures are compatible, the non-dissipative part
                   of the inverse matrix of response coefficients turns
                   out to be immune to dephasing. We give three examples
                   of physical systems whose quantum states induce
                   compatible metric and symplectic structures on
                   control space: qubit, coherent states and a model of
                   the integer quantum Hall effect.},
  doi =           {10.1088/1367-2630/13/5/053042},
  issn =          {1367-2630},
  url =           {http://stacks.iop.org/1367-2630/13/i=5/a=053042?
                  key=crossref.30aead48e72045361d8e00c569da5d56},
}

@article{Bardyn2013,
  author =        {Bardyn, C-E and Baranov, M. A. and Kraus, C. V. and
                   Rico, E. and
                   $\backslash$.{\{}I{\}}mamo$\backslash$u{\{}g{\}}lu, A and
                   Zoller, P. and Diehl, S.},
  journal =       {New J. Phys.},
  month =         {aug},
  number =        {8},
  pages =         {085001},
  title =         {{Topology by dissipation}},
  volume =        {15},
  year =          {2013},
  abstract =      {Topological states of fermionic matter can be induced
                   by means of a suitably engineered dissipative
                   dynamics. Dissipation then does not occur as a
                   perturbation, but rather as the main resource for
                   many-body dynamics, providing a targeted cooling into
                   topological phases starting from arbitrary initial
                   states. We explore the concept of topological order
                   in this setting, developing and applying a general
                   theoretical framework based on the system density
                   matrix that replaces the wave function appropriate
                   for the discussion of Hamiltonian ground-state
                   physics. We identify key analogies and differences to
                   the more conventional Hamiltonian scenario.
                   Differences essentially arise from the fact that the
                   properties of the spectrum and of the state of the
                   system are not as tightly related as in the
                   Hamiltonian context. We provide a symmetry-based
                   topological classification of bulk steady states and
                   identify the classes that are achievable by means of
                   quasi-local dissipative processes driving into
                   superfluid paired states. We also explore the fate of
                   the bulk-edge correspondence in the dissipative
                   setting and demonstrate the emergence of Majorana
                   edge modes. We illustrate our findings in one-and
                   two-dimensional models that are experimentally
                   realistic in the context of cold atoms.},
  doi =           {10.1088/1367-2630/15/8/085001},
  isbn =          {1367-2630},
  issn =          {1367-2630},
  url =           {http://stacks.iop.org/1367-2630/15/i=8/a=085001?
                  key=crossref.dbfc132c3a50871fe00070d6baa253c4},
}

@article{Huang2014,
  author =        {Huang, Zhoushen and Arovas, Daniel P.},
  journal =       {Phys. Rev. Lett.},
  month =         {aug},
  number =        {7},
  pages =         {076407},
  title =         {{Topological Indices for Open and Thermal Systems Via
                   Uhlmann's Phase}},
  volume =        {113},
  year =          {2014},
  abstract =      {Two-dimensional topological phases are characterized
                   by TKNN integers, which classify Bloch energy bands
                   or groups of Bloch bands. However, quantization does
                   not survive thermal averaging or dephasing to mixed
                   states. We show that using Uhlmann's parallel
                   transport for density matrices (Rep. Math. Phys. 24,
                   229 (1986)), an integer classification of topological
                   phases can be defined for a finite generalized
                   temperature {\$}T{\$} or dephasing Lindbladian. This
                   scheme reduces to the familiar TKNN classification
                   for {\$}T{\textless}T{\_}{\{}{\{}\backslashrm
                   c{\}},1{\}}{\$}, becomes trivial for
                   {\$}T{\textgreater}T{\_}{\{}{\{}\backslashrm
                   c{\}},2{\}}{\$}, and exhibits a `gapless'
                   intermediate regime where topological indices are not
                   well-defined. We demonstrate these ideas in detail,
                   applying them to Haldane's honeycomb lattice model
                   and the Bernevig-Hughes-Zhang model, and we comment
                   on their generalization to multi-band Chern
                   insulators.},
  doi =           {10.1103/PhysRevLett.113.076407},
  issn =          {0031-9007},
  url =           {http://link.aps.org/doi/10.1103/
                  PhysRevLett.113.076407 https://link.aps.org/doi/10.1103/
                  PhysRevLett.113.076407},
}

@article{Viyuela2014,
  author =        {Viyuela, O. and Rivas, A. and Martin-Delgado, M. A.},
  journal =       {Phys. Rev. Lett.},
  month =         {apr},
  number =        {13},
  pages =         {130401},
  title =         {{Uhlmann Phase as a Topological Measure for
                   One-Dimensional Fermion Systems}},
  volume =        {112},
  year =          {2014},
  abstract =      {We introduce the Uhlmann geometric phase as a tool to
                   characterize symmetry-protected topological phases in
                   1D fermion systems, such as topological insulators
                   and superconductors. Since this phase is formulated
                   for general mixed quantum states, it provides a way
                   to extend topological properties to finite
                   temperature situations. We illustrate these ideas
                   with some paradigmatic models and find that there
                   exists a critical temperature {\$}T{\_}c{\$} at which
                   the Uhlmann phase goes discontinuously and abruptly
                   to zero. This stands as a borderline between two
                   different topological phases as a function of the
                   temperature. Furthermore, at small temperatures we
                   recover the usual notion of topological phase in
                   fermion systems.},
  doi =           {10.1103/PhysRevLett.112.130401},
  isbn =          {0031-9007$\backslash$r1079-7114},
  issn =          {0031-9007},
  url =           {https://link.aps.org/doi/10.1103/PhysRevLett.112.130401},
}

@article{Viyuela2014a,
  author =        {Viyuela, O. and Rivas, A. and Martin-Delgado, M. a.},
  journal =       {Phys. Rev. Lett.},
  number =        {7},
  pages =         {076408},
  title =         {{Two-Dimensional Density-Matrix Topological Fermionic
                   Phases: Topological Uhlmann Numbers}},
  volume =        {113},
  year =          {2014},
  abstract =      {We construct a topological invariant that classifies
                   density matrices of symmetry-protected topological
                   orders in 2D fermionic systems. As it is constructed
                   out of the previously introduced Uhlmann phase, we
                   refer to it as the topological Uhlmann number
                   {\$}{\{}\backslashrm n{\}}{\_}{\{}\backslashrm
                   U{\}}{\$}. With it, we study thermal topological
                   phases in several 2D models of topological insulators
                   and superconductors, computing phase diagrams where
                   the temperature {\$}T{\$} is on equal footing with
                   the coupling constants in the Hamiltonian. Moreover,
                   we find novel thermal-topological transitions between
                   two non-trivial phases in a model with high Chern
                   numbers. At small temperature we recover the standard
                   topological phases as the Uhlmann number approaches
                   to the Chern number.},
  doi =           {10.1103/PhysRevLett.113.076408},
  isbn =          {0031-9007$\backslash$r1079-7114},
  issn =          {0031-9007},
  url =           {http://link.aps.org/doi/10.1103/PhysRevLett.113.076408},
}

@article{Budich2015a,
  author =        {Budich, Jan Carl and Diehl, Sebastian},
  journal =       {Phys. Rev. B},
  month =         {apr},
  number =        {16},
  pages =         {165140},
  title =         {{Topology of density matrices}},
  volume =        {91},
  year =          {2015},
  abstract =      {We investigate topological properties of density
                   matrices motivated by the question to what extent
                   phenomena like topological insulators and
                   superconductors can be generalized to mixed states in
                   the framework of open quantum systems. The notion of
                   geometric phases has been extended from pure to mixed
                   states by Uhlmann in [Rep. Math. Phys. 24, 229
                   (1986)], where an emergent gauge theory over the
                   density matrices based on their pure-state
                   representation in a larger Hilbert space has been
                   reported. However, since the uniquely defined square
                   root {\$}\backslashsqrt{\{}\backslashrho{\}}{\$} of a
                   density matrix {\$}\backslashrho{\$} provides a
                   global gauge, this construction is always
                   topologically trivial. Here, we study a more
                   restrictive gauge structure which can be
                   topologically non-trivial and is capable of resolving
                   homotopically distinct mappings of density matrices
                   subject to various spectral constraints. Remarkably,
                   in this framework, topological invariants can be
                   directly defined and calculated for mixed states. In
                   the limit of pure states, the well known system of
                   topological invariants for gapped band structures at
                   zero temperature is reproduced. We compare our
                   construction with recent approaches to Chern
                   insulators at finite temperature.},
  doi =           {10.1103/PhysRevB.91.165140},
  issn =          {1098-0121},
  url =           {https://link.aps.org/doi/10.1103/PhysRevB.91.165140},
}

@article{Linzner2016,
  author =        {Linzner, D. and Wawer, L. and Grusdt, F. and
                   Fleischhauer, M.},
  journal =       {Phys. Rev. B},
  month =         {nov},
  number =        {20},
  pages =         {201105},
  title =         {{Reservoir-induced Thouless pumping and
                   symmetry-protected topological order in open quantum
                   chains}},
  volume =        {94},
  year =          {2016},
  abstract =      {We discuss an open-system analogue of a topological
                   Thouless pump in the steady state of a
                   one-dimensional spin lattice driven by Markovian
                   reservoirs. Periodic variations in a two-dimensional
                   parameter space are shown to lead to quantized
                   transport through the lattice. On an extremal path in
                   parameter space the steady state is pure state and
                   coincides with the ground state of the Rice-Mele
                   Hamiltonian for fermions at half filling. Here the
                   quantized transport can be associated with a
                   topological invariant based on geometric phases, the
                   Chern number. On a more general path, where the
                   steady state is mixed, we introduce the winding of
                   the many-body polarization as a generalized
                   topological invariant. We show that it applies to
                   open quantum systems and includes the effects of
                   interactions and moderate particle-number
                   fluctuations. The winding of polarization, which
                   characterizes the Thouless pump is robust against
                   Hamiltonian perturbations as well as dephasing and
                   particle losses.},
  doi =           {10.1103/PhysRevB.94.201105},
  issn =          {2469-9950},
  url =           {https://link.aps.org/doi/10.1103/PhysRevB.94.201105},
}

@article{Mera2017,
  author =        {Mera, Bruno and Vlachou, Chrysoula and
                   Paunkovi{\'{c}}, Nikola and Vieira, V{\'{i}}tor R.},
  journal =       {Phys. Rev. Lett.},
  month =         {jul},
  number =        {1},
  pages =         {015702},
  title =         {{Uhlmann Connection in Fermionic Systems Undergoing
                   Phase Transitions}},
  volume =        {119},
  year =          {2017},
  doi =           {10.1103/PhysRevLett.119.015702},
  issn =          {0031-9007},
  url =           {http://link.aps.org/doi/10.1103/PhysRevLett.119.015702},
}

@article{Grusdt2017,
  author =        {Grusdt, F.},
  journal =       {Phys. Rev. B},
  month =         {feb},
  number =        {7},
  pages =         {075106},
  title =         {{Topological order of mixed states in correlated
                   quantum many-body systems}},
  volume =        {95},
  year =          {2017},
  abstract =      {Topological order has become a new paradigm to
                   distinguish ground states of interacting many-body
                   systems without conventional long-range order. Here
                   we discuss possible extensions of this concept to
                   density matrices describing statistical ensembles.
                   For a large class of quasi-thermal states, which can
                   be realized as thermal states of some quasi-local
                   Hamiltonian, we generalize earlier definitions of
                   density matrix topology to generic many-body systems
                   with strong correlations. We point out that the
                   robustness of topological order, defined as a pattern
                   of long-range entanglement, depends crucially on the
                   perturbations under consideration. While it is
                   intrinsically protected against local perturbations
                   of arbitrary strength in an infinite closed quantum
                   system, purely local perturbations can destroy
                   topological order in open systems coupled to baths if
                   the coupling is sufficiently strong. We discuss our
                   classification scheme using the finite-temperature
                   quantum Hall states and point out that the classical
                   Hall effect can be understood as a finite temperature
                   topological phase.},
  doi =           {10.1103/PhysRevB.95.075106},
  issn =          {2469-9950},
  url =           {https://link.aps.org/doi/10.1103/PhysRevB.95.075106},
}

@article{Bardyn2018,
  author =        {Bardyn, Charles-Edouard and Wawer, Lukas and
                   Altland, Alexander and Fleischhauer, Michael and
                   Diehl, Sebastian},
  journal =       {Phys. Rev. X},
  month =         {feb},
  number =        {1},
  pages =         {011035},
  publisher =     {American Physical Society},
  title =         {{Probing the Topology of Density Matrices}},
  volume =        {8},
  year =          {2018},
  abstract =      {The mixedness of a quantum state is usually seen as
                   an adversary to topological quantization of
                   observables. For example, exact quantization of the
                   charge transported in a so-called Thouless adiabatic
                   pump is lifted at any finite temperature in
                   symmetry-protected topological insulators. Here, we
                   show that certain directly observable many-body
                   correlators preserve the integrity of topological
                   invariants for mixed Gaussian quantum states in one
                   dimension. Our approach relies on the expectation
                   value of the many-body momentum-translation operator,
                   and leads to a physical observable --- the "ensemble
                   geometric phase" (EGP) --- which represents a bona
                   fide geometric phase for mixed quantum states, in the
                   thermodynamic limit. In cyclic protocols, the EGP
                   provides a topologically quantized observable which
                   detects encircled spectral singularities
                   ("purity-gap" closing points) of density matrices.
                   While we identify the many-body nature of the EGP as
                   a key ingredient, we propose a conceptually simple,
                   interferometric setup to directly measure the latter
                   in experiments with mesoscopic ensembles of ultracold
                   atoms.},
  doi =           {10.1103/PhysRevX.8.011035},
  issn =          {2160-3308},
  url =           {http://arxiv.org/abs/1706.02741 https://link.aps.org/doi/
                  10.1103/PhysRevX.8.011035},
}

@article{Uhlmann1986,
  author =        {Uhlmann, Armin},
  journal =       {Reports Math. Phys.},
  month =         {oct},
  number =        {2},
  pages =         {229--240},
  title =         {{Parallel transport and “quantum holonomy” along
                   density operators}},
  volume =        {24},
  year =          {1986},
  doi =           {10.1016/0034-4877(86)90055-8},
  issn =          {00344877},
  url =           {http://linkinghub.elsevier.com/retrieve/pii/
                  0034487786900558},
}

@article{Uhlmann1991,
  author =        {Uhlmann, Armin},
  journal =       {Lett. Math. Phys.},
  month =         {mar},
  number =        {3},
  pages =         {229--236},
  title =         {{A gauge field governing parallel transport along
                   mixed states}},
  volume =        {21},
  year =          {1991},
  abstract =      {At first, a short account is given of some basic
                   notations and results on parallel transport along
                   mixed states. A new connection form (gauge field) is
                   introduced to give a geometric meaning to the concept
                   of parallelity in the theory of density operators.},
  doi =           {10.1007/BF00420373},
  issn =          {0377-9017},
  url =           {http://link.springer.com/10.1007/BF00420373},
}

@article{Carollo2018,
  author =        {Carollo, Angelo and Spagnolo, Bernardo and
                   Valenti, Davide},
  journal =       {Sci. Rep.},
  number =        {1},
  pages =         {9852},
  title =         {{Uhlmann curvature in dissipative phase transitions}},
  volume =        {8},
  year =          {2018},
  abstract =      {A novel approach based on the Uhlmann curvature is
                   introduced for the investigation of non-equilibrium
                   steady-state quantum phase transitions (NESS-QPTs).
                   Equilibrium phase transitions fall invariably into
                   two markedly non-overlapping categories: classical
                   phase transitions and quantum phase transitions.
                   NESS-QPTs offer a unique arena where such a
                   distinction fades off. We propose a method to reveal
                   and quantitatively assess the quantum character of
                   such critical phenomena. We apply this tool to a
                   paradigmatic class of lattice fermion systems with
                   local reservoirs, characterised by Gaussian
                   non-equilibrium steady states. The relations between
                   the behaviour of the Uhlmann curvature, the
                   divergence of the correlation length, the character
                   of the criticality and the dissipative gap are
                   demonstrated. We argue that this tool can shade light
                   upon the nature of non equilibrium steady state
                   criticality in particular with regard to the role
                   played by quantum vs classical fluctuations.},
  doi =           {10.1038/s41598-018-27362-9},
  issn =          {2045-2322},
  url =           {https://doi.org/10.1038/s41598-018-27362-9},
}

@article{Carollo2018a,
  author =        {Carollo, Angelo and Spagnolo, Bernardo and
                   Valenti, Davide},
  journal =       {Entropy},
  month =         {jun},
  number =        {7},
  pages =         {485},
  title =         {{Symmetric Logarithmic Derivative of Fermionic
                   Gaussian States}},
  volume =        {20},
  year =          {2018},
  doi =           {10.3390/e20070485},
  issn =          {1099-4300},
  url =           {http://www.mdpi.com/1099-4300/20/7/485},
}

@article{Leonforte2018,
  author =        {Leonforte, Luca and Valenti, Davide and
                   Spagnolo, Bernardo and Carollo, Angelo},
  month =         {jun},
  title =         {{Uhlmann number in translational invariant systems}},
  year =          {2018},
  abstract =      {We define the Uhlmann number as an extension of the
                   Chern number, and we use this quantity to describe
                   the topology of 2D translational invariant fermionic
                   systems at finite temperature. We consider two
                   paradigmatic systems, representing classes of systems
                   that can have non-trivial topology characterized by
                   the Chern number, and we study the changes in their
                   topology through the Uhlmann number. At low
                   temperature we find the topological phase transitions
                   predicted by the Chern number. However, at higher
                   temperature, by using the Uhlmann number, we find a
                   cross-over behaviour without any criticalities. Then,
                   we find a relation in a general system between the
                   mean Uhlmann curvature and the dynamical
                   susceptibility, which gives a hint on how to measure
                   the mean Uhlmann curvature. We also link the Uhlmann
                   number to the dynamical conductivity of topological
                   insulators and superconductors, which extends the
                   TKNN formula to finite temperature. Finally, we
                   relate the mean Uhlmann curvature in the electric
                   field parameter space to the Uhlmann number, whose
                   relation can have an important meaning in the
                   multi-parameter estimation problem.},
  url =           {http://arxiv.org/abs/1806.08592},
}

@article{Magazzu2015,
  author =        {Magazz{\`{u}}, Luca and Valenti, Davide and
                   Carollo, Angelo and Spagnolo, Bernardo},
  journal =       {Entropy},
  number =        {4},
  pages =         {2341--2354},
  publisher =     {MDPI AG},
  title =         {{Multi-state quantum dissipative dynamics in
                   sub-ohmic environment: The strong coupling regime}},
  volume =        {17},
  year =          {2015},
  abstract =      {We study the dissipative quantum dynamics and the
                   asymptotic behavior of a particle in a bistable
                   potential interacting with a sub-Ohmic broadband
                   environment. The reduced dynamics, in the
                   intermediate to strong dissipation regime, is
                   obtained beyond the two-level system approximation by
                   using a real-time path integral approach. We find a
                   crossover dynamic regime with damped intra-well
                   oscillations and incoherent tunneling and a
                   completely incoherent regime at strong damping.
                   Moreover, a nonmonotonic behavior of the left/right
                   well population difference is found as a function of
                   the damping strength.},
}

@article{Spagnolo2018,
  author =        {Spagnolo, Bernardo and Carollo, Angelo and
                   Valenti, Davide},
  journal =       {Entropy},
  month =         {mar},
  number =        {4},
  pages =         {226},
  title =         {{Enhancing Metastability by Dissipation and Driving
                   in an Asymmetric Bistable Quantum System}},
  volume =        {20},
  year =          {2018},
  abstract =      {{\textcopyright} 2018 by the authors. The stabilizing
                   effect of quantum fluctuations on the escape process
                   and the relaxation dynamics from a quantum metastable
                   state are investigated. Specifically, the quantum
                   dynamics of a multilevel bistable system coupled to a
                   bosonic Ohmic thermal bath in strong dissipation
                   regime is analyzed. The study is performed by a
                   non-perturbative method based on the real-time path
                   integral approach of the Feynman-Vernon influence
                   functional. We consider a strongly asymmetric double
                   well potential with and without a monochromatic
                   external driving, and with an out-of-equilibrium
                   initial condition. In the absence of driving we
                   observe a nonmonotonic behavior of the escape time
                   from the metastable region, as a function both of the
                   system-bath coupling coefficient and the temperature.
                   This indicates a stabilizing effect of the quantum
                   fluctuations. In the presence of driving our findings
                   indicate that, as the coupling coefficient $\gamma$
                   increases, the escape time, initially controlled by
                   the external driving, shows resonant peaks and dips,
                   becoming frequency-independent for higher $\gamma$
                   values. Moreover, the escape time from the metastable
                   state displays a nonmonotonic behavior as a function
                   of the temperature, the frequency of the driving, and
                   the thermal-bath coupling, which indicates the
                   presence of a quantum noise enhanced stability
                   phenomenon. Finally, we investigate the role of
                   different spectral densities, both in sub-Ohmic and
                   super-Ohmic dissipation regime and for different
                   cutoff frequencies, on the relaxation dynamics from
                   the quantum metastable state. The results obtained
                   indicate that, in the crossover dynamical regime
                   characterized by damped intrawell oscillations and
                   incoherent tunneling, the spectral properties of the
                   thermal bath influence non-trivially the short time
                   behavior and the time scales of the relaxation
                   dynamics from the metastable state.},
  doi =           {10.3390/e20040226},
  issn =          {1099-4300},
  url =           {http://www.mdpi.com/1099-4300/20/4/226},
}

@article{Valenti2018,
  author =        {Valenti, Davide and Carollo, Angelo and
                   Spagnolo, Bernardo},
  journal =       {Phys. Rev. A},
  month =         {apr},
  number =        {4},
  pages =         {042109},
  title =         {{Stabilizing effect of driving and dissipation on
                   quantum metastable states}},
  volume =        {97},
  year =          {2018},
  doi =           {10.1103/PhysRevA.97.042109},
  issn =          {2469-9926},
  url =           {https://link.aps.org/doi/10.1103/PhysRevA.97.042109},
}

@article{Spagnolo2018a,
  author =        {Spagnolo, Bernardo and Carollo, Angelo and
                   Valenti, Davide},
  journal =       {Eur. Phys. J. Spec. Top.},
  month =         {sep},
  number =        {3-4},
  pages =         {379--420},
  title =         {{Stabilization by dissipation and stochastic resonant
                   activation in quantum metastable systems}},
  volume =        {227},
  year =          {2018},
  doi =           {10.1140/epjst/e2018-00121-x},
  issn =          {1951-6355},
  url =           {https://link.springer.com/article/
                  10.1140{\%}2Fepjst{\%}2Fe2018-00121-x http://
                  link.springer.com/10.1140/epjst/e2018-00121-x},
}

@article{Guarcello2015,
  author =        {Guarcello, Claudio and Valenti, Davide and
                   Carollo, Angelo and Spagnolo, Bernardo},
  journal =       {J. Stat. Mech. Theory Exp.},
  month =         {may},
  number =        {5},
  pages =         {054012},
  publisher =     {IOP Publishing},
  title =         {{Effects of L$\backslash$'evy noise on the dynamics
                   of sine-Gordon solitons in long Josephson junctions}},
  volume =        {2016},
  year =          {2016},
  doi =           {10.1088/1742-5468/2016/05/054012},
  issn =          {1742-5468},
  url =           {http://arxiv.org/abs/1511.04899 http://stacks.iop.org/1742-
                  5468/2016/i=5/a=054012?
                  key=crossref.48e7f7f504b019713822c481ca8bac97},
}

@article{Spagnolo2016,
  author =        {Spagnolo, Bernardo and Guarcello, Claudio and
                   Magazz{\`{u}}, Luca and Carollo, Angelo and
                   {Persano Adorno}, Dominique and Valenti, Davide},
  journal =       {Entropy},
  month =         {dec},
  number =        {1},
  pages =         {20},
  title =         {{Nonlinear Relaxation Phenomena in Metastable
                   Condensed Matter Systems}},
  volume =        {19},
  year =          {2016},
  abstract =      {{\textcopyright} 2016 by the authors. Nonlinear
                   relaxation phenomena in three different systems of
                   condensed matter are investigated. (i) First, the
                   phase dynamics in Josephson junctions is analyzed.
                   Specifically, a
                   superconductor-graphene-superconductor (SGS) system
                   exhibits quantum metastable states, and the average
                   escape time from these metastable states in the
                   presence of Gaussian and correlated fluctuations is
                   calculated, accounting for variations in the the
                   noise source intensity and the bias frequency.
                   Moreover, the transient dynamics of a long-overlap
                   Josephson junction (JJ) subject to thermal
                   fluctuations and non-Gaussian noise sources is
                   investigated. Noise induced phenomena are observed,
                   such as the noise enhanced stability and the
                   stochastic resonant activation. (ii) Second, the
                   electron spin relaxation process in a n-type GaAs
                   bulk driven by a fluctuating electric field is
                   investigated. In particular, by using a Monte Carlo
                   approach, we study the influence of a random
                   telegraph noise on the spin polarized transport. Our
                   findings show the possibility to raise the spin
                   relaxation length by increasing the amplitude of the
                   external fluctuations. Moreover, we find that,
                   crucially, depending on the value of the external
                   field strength, the electron spin depolarization
                   length versus the noise correlation time increases up
                   to a plateau. (iii) Finally, the stabilization of
                   quantum metastable states by dissipation is
                   presented. Normally, quantum fluctuations enhance the
                   escape from metastable states in the presence of
                   dissipation. We show that dissipation can enhance the
                   stability of a quantum metastable system, consisting
                   of a particle moving in a strongly asymmetric double
                   well potential, interacting with a thermal bath. We
                   find that the escape time from the metastable region
                   has a nonmonotonic behavior versus the system- bath
                   coupling and the temperature, producing a stabilizing
                   effect.},
  doi =           {10.3390/e19010020},
  issn =          {1099-4300},
  url =           {http://www.mdpi.com/1099-4300/19/1/20},
}

@article{Spagnolo2015,
  author =        {Spagnolo, B. and Valenti, D. and Guarcello, C. and
                   Carollo, A. and {Persano Adorno}, D. and Spezia, S. and
                   Pizzolato, N. and {Di Paola}, B.},
  journal =       {Chaos, Solitons and Fractals},
  pages =         {412--424},
  publisher =     {Elsevier Ltd.},
  title =         {{Noise-induced effects in nonlinear relaxation of
                   condensed matter systems}},
  volume =        {81},
  year =          {2015},
  abstract =      {Noise-induced phenomena characterise the nonlinear
                   relaxation of nonequilibrium physical systems towards
                   equilibrium states. Often, this relaxation process
                   proceeds through metastable states and the noise can
                   give rise to resonant phenomena with an enhancement
                   of lifetime of these states or some coherent state of
                   the condensed matter system considered. In this paper
                   three noise induced phenomena, namely the noise
                   enhanced stability, the stochastic resonant
                   activation and the noise-induced coherence of
                   electron spin, are reviewed in the nonlinear
                   relaxation dynamics of three different systems of
                   condensed matter: (i) a long-overlap Josephson
                   junction (JJ) subject to thermal fluctuations and
                   non-Gaussian, L{\'{e}}vy distributed, noise sources;
                   (ii) a graphene-based Josephson junction subject to
                   thermal fluctuations; (iii) electrons in a n-type
                   GaAs crystal driven by a fluctuating electric field.
                   In the first system, we focus on the switching events
                   from the superconducting metastable state to the
                   resistive state, by solving the perturbed stochastic
                   sine-Gordon equation. Nonmonotonic behaviours of the
                   mean switching time versus the noise intensity,
                   frequency of the external driving, and length of the
                   junction are obtained. Moreover, the influence of the
                   noise induced solitons on the mean switching time
                   behaviour is shown. In the second system, noise
                   induced phenomena are observed, such as noise
                   enhanced stability (NES) and stochastic resonant
                   activation (SRA). In the third system, the spin
                   polarised transport in GaAs is explored in two
                   different scenarios, i.e. in the presence of Gaussian
                   correlated fluctuations or symmetric dichotomous
                   noise. Numerical results indicate an increase of the
                   electron spin lifetime by rising the strength of the
                   random fluctuating component. Furthermore, our
                   findings for the electron spin depolarization time as
                   a function of the noise correlation time point out
                   (i) a non-monotonic behaviour with a maximum in the
                   case of Gaussian correlated fluctuations, (ii) an
                   increase up to a plateau in the case of dichotomous
                   noise. The noise enhances the coherence of the spin
                   relaxation process.},
  doi =           {10.1016/j.chaos.2015.07.023},
  issn =          {09600779},
  url =           {http://dx.doi.org/10.1016/j.chaos.2015.07.023},
}

@article{Spagnolo2012,
  author =        {Spagnolo, B and Caldara, P and {La Cognata}, A and
                   Valenti, D and Fiasconaro, A and Dubkov, A A and
                   Falci, G},
  journal =       {Int. J. Mod. Phys. B},
  month =         {may},
  number =        {12},
  pages =         {1241006},
  publisher =     {World Scientific Publishing Company},
  title =         {{The Bistable Potential: An Archetype For Classical
                   And Quantum Systems}},
  volume =        {26},
  year =          {2012},
  abstract =      {In this work we analyze the transient dynamics of
                   three different classical and quantum systems. First,
                   we consider a classical Brownian particle moving in
                   an asymmetric bistable potential, subject to a
                   multiplicative and additive noise source. We
                   investigate the role of these two noise sources on
                   the life time of the metastable state. A nonmonotonic
                   behavior of the lifetime as a function of both
                   additive and multiplicative noise intensities is
                   found, revealing the phenomenon of noise enhanced
                   stability. Afterward, by using a Lotka�Volterra
                   model, the dynamics of two competing species in the
                   presence of L{\'{e}}vy noise sources is analyzed.
                   Quasiperiodic oscillations and stochastic resonance
                   phenomenon in the dynamics of the competing species
                   are found. Finally the dynamics of a quantum particle
                   subject to an asymmetric bistable potential and
                   interacting with a thermal reservoir is investigated.
                   We use the Caldeira�Leggett model and the approach
                   of the Feynman�Vernon functional in discrete
                   variable representati...},
  doi =           {10.1142/S0217979212410068},
  issn =          {0217-9792},
  url =           {http://www.worldscientific.com/doi/abs/10.1142/
                  S0217979212410068},
}

@article{He2018,
  author =        {He, Yan and Guo, Hao and Chien, Chih-Chun},
  journal =       {Phys. Rev. B},
  month =         {jun},
  number =        {23},
  pages =         {235141},
  publisher =     {American Physical Society},
  title =         {{Thermal Uhlmann-Chern number from the Uhlmann
                   connection for extracting topological properties of
                   mixed states}},
  volume =        {97},
  year =          {2018},
  abstract =      {The Berry phase is a geometric phase of a pure state
                   when the system is adiabatically transported along a
                   loop in its parameter space. The concept of geometric
                   phase has been generalized to mixed states by the so
                   called Uhlmann phase. However, the Uhlmann phase is
                   constructed from the Uhlmann connection that
                   possesses a well defined global section. This
                   property implies that the Uhlmann connection is
                   topologically trivial and as a consequence, the
                   corresponding Chern character vanishes. We propose
                   modified Chern character whose integral gives the
                   thermal Uhlmann Chern number, which is related to the
                   winding number of the mapping defined by the
                   Hamiltonian. Therefore, the thermal Uhlmann Chern
                   number reflects the topological properties of the
                   underlying Hamiltonian of a mixed state. By including
                   the temperature dependence in the volume integral, we
                   also introduce the non-topological thermal Uhlmann
                   Chern number which varies with temperature but is not
                   quantized at finite temperatures. We illustrate the
                   applications to a two-band model and a degenerate
                   four-band model.},
  doi =           {10.1103/PhysRevB.97.235141},
  issn =          {2469-9950},
  url =           {https://link.aps.org/doi/10.1103/PhysRevB.97.235141},
}

@inproceedings{Preskill1997,
  author =        {Shor, P.W.},
  booktitle =     {Proc. 37th Conf. Found. Comput. Sci.},
  pages =         {56--65},
  publisher =     {IEEE Comput. Soc. Press},
  title =         {{Fault-tolerant quantum computation}},
  year =          {1997},
  abstract =      {The discovery of quantum error correction has greatly
                   improved the long-term prospects for quantum
                   computing technology. Encoded quantum information can
                   be protected from errors that arise due to
                   uncontrolled interactions with the environment, or
                   due to imperfect implementations of quantum logical
                   operations. Recovery from errors can work effectively
                   even if occasional mistakes occur during the recovery
                   procedure. Furthermore, encoded quantum information
                   can be processed without serious propagation of
                   errors. In principle, an arbitrarily long quantum
                   computation can be performed reliably, provided that
                   the average probability of error per gate is less
                   than a certain critical value, the accuracy
                   threshold. It may be possible to incorporate
                   intrinsic fault tolerance into the design of quantum
                   computing hardware, perhaps by invoking topological
                   Aharonov-Bohm interactions to process quantum
                   information.},
  doi =           {10.1109/SFCS.1996.548464},
  isbn =          {0-8186-7594-2},
  issn =          {0272-5428},
  url =           {http://arxiv.org/abs/quant-ph/9712048 http://
                  ieeexplore.ieee.org/document/548464/},
}

@article{Kitaev2003,
  author =        {Kitaev, A.Yu.},
  journal =       {Ann. Phys. (N. Y).},
  month =         {jan},
  number =        {1},
  pages =         {2--30},
  title =         {{Fault-tolerant quantum computation by anyons}},
  volume =        {303},
  year =          {2003},
  abstract =      {A two-dimensional quantum system with anyonic
                   excitations can be considered as a quantum computer.
                   Unitary transformations can be performed by moving
                   the excitations around each other. Measurements can
                   be performed by joining excitations in pairs and
                   observing the result of fusion. Such computation is
                   fault-tolerant by its physical nature. ?? 2002
                   Elsevier Science (USA). All rights reserved.},
  doi =           {10.1016/S0003-4916(02)00018-0},
  isbn =          {0003-4916},
  issn =          {00034916},
  url =           {http://linkinghub.elsevier.com/retrieve/pii/
                  S0003491602000180},
}

@article{Kitaev2009,
  author =        {Kitaev, Alexei},
  journal =       {AIP Conf. Proc.},
  pages =         {22--30},
  title =         {{Periodic table for topological insulators and
                   superconductors}},
  volume =        {1134},
  year =          {2009},
  abstract =      {Gapped phases of noninteracting fermions, with and
                   without charge conservation and time‐reversal
                   symmetry, are classified using Bott periodicity. The
                   symmetry and spatial dimension determines a general
                   universality class, which corresponds to one of the 2
                   types of complex and 8 types of real Clifford
                   algebras. The phases within a given class are further
                   characterized by a topological invariant, an element
                   of some Abelian group that can be 0, Z, or Z2. The
                   interface between two infinite phases with different
                   topological numbers must carry some gapless mode.
                   Topological properties of finite systems are
                   described in terms of K‐homology. This
                   classification is robust with respect to disorder,
                   provided electron states near the Fermi energy are
                   absent or localized. In some cases (e.g., integer
                   quantum Hall systems) the K‐theoretic
                   classification is stable to interactions, but a
                   counterexample is also given.},
  doi =           {10.1063/1.3149495},
  isbn =          {9780735406711},
  issn =          {0094243X},
}

@article{Kitaev2006,
  author =        {Kitaev, Alexei},
  journal =       {Ann. Phys. (N. Y).},
  number =        {1},
  pages =         {2--111},
  title =         {{Anyons in an exactly solved model and beyond}},
  volume =        {321},
  year =          {2006},
  abstract =      {A spin-1/2 system on a honeycomb lattice is studied.
                   The interactions between nearest neighbors are of XX,
                   YY or ZZ type, depending on the direction of the
                   link; different types of interactions may differ in
                   strength. The model is solved exactly by a reduction
                   to free fermions in a static ℤ2 gauge field. A
                   phase diagram in the parameter space is obtained. One
                   of the phases has an energy gap and carries
                   excitations that are Abelian anyons. The other phase
                   is gapless, but acquires a gap in the presence of
                   magnetic field. In the latter case excitations are
                   non-Abelian anyons whose braiding rules coincide with
                   those of conformal blocks for the Ising model. We
                   also consider a general theory of free fermions with
                   a gapped spectrum, which is characterized by a
                   spectral Chern number v. The Abelian and non-Abelian
                   phases of the original model correspond to v = 0 and
                   v = ±1, respectively. The anyonic properties of
                   excitation depend on v mod 16, whereas v itself
                   governs edge thermal transport. The paper also
                   provides mathematical background on anyons as well as
                   an elementary theory of Chern number for
                   quasidiagonal matrices. {\textcopyright} 2005
                   Elsevier Inc. All rights reserved.},
  doi =           {10.1016/j.aop.2005.10.005},
  isbn =          {0003-4916},
  issn =          {00034916},
}

@article{Kells2009,
  author =        {Kells, G. and Slingerland, J. K. and Vala, J.},
  journal =       {Phys. Rev. B - Condens. Matter Mater. Phys.},
  number =        {12},
  pages =         {1--10},
  title =         {{Description of Kitaev's honeycomb model with
                   toric-code stabilizers}},
  volume =        {80},
  year =          {2009},
  abstract =      {We present a solution of Kitaev's spin model on the
                   honeycomb lattice and of related topologically
                   ordered spin models. We employ a Jordan-Wigner type
                   fermionization and find that the Hamiltonian takes a
                   BCS type form, allowing the system to be solved by
                   Bogoliubov transformation. Our fermionization does
                   not employ non-physical auxiliary degrees of freedom
                   and the eigenstates we obtain are completely explicit
                   in terms of the spin variables. The ground-state is
                   obtained as a BCS condensate of fermion pairs over a
                   vacuum state which corresponds to the toric code
                   state with the same vorticity. We show in detail how
                   to calculate all eigenstates and eigenvalues of the
                   model on the torus. In particular, we find that the
                   topological degeneracy on the torus descends directly
                   from that of the toric code, which now supplies four
                   vacua for the fermions, one for each choice of
                   periodic vs. anti-periodic boundary conditions. The
                   reduction of the degeneracy in the non-Abelian phase
                   of the model is seen to be due to the vanishing of
                   one of the corresponding candidate BCS ground-states
                   in that phase. This occurs in particular in the fully
                   periodic vortex-free sector. The true ground-state in
                   this sector is exhibited and shown to be gapped away
                   from the three partially anti-periodic ground-states
                   whenever the non-Abelian phase is gapped.},
  doi =           {10.1103/PhysRevB.80.125415},
  issn =          {10980121},
}

@article{Kells2008,
  author =        {Kells, G. and Bolukbasi, A. T. and Lahtinen, V. and
                   Slingerland, J. K. and Pachos, J. K. and Vala, J.},
  journal =       {Phys. Rev. Lett.},
  month =         {dec},
  number =        {24},
  pages =         {240404},
  title =         {{Topological Degeneracy and Vortex Manipulation in
                   Kitaev's Honeycomb Model}},
  volume =        {101},
  year =          {2008},
  abstract =      {The classification of loop symmetries in Kitaev's
                   honeycomb lattice model provides a natural framework
                   to study the Abelian topological degeneracy. We
                   derive a perturbative low-energy effective
                   Hamiltonian that is valid to all orders of the
                   expansion and for all possible toroidal
                   configurations. Using this form we demonstrate at
                   what order the system's topological degeneracy is
                   lifted by finite size effects and note that in the
                   thermodynamic limit it is robust to all orders.
                   Further, we demonstrate that the loop symmetries
                   themselves correspond to the creation, propagation,
                   and annihilation of fermions. We note that these
                   fermions, made from pairs of vortices, can be moved
                   with no additional energy cost.},
  doi =           {10.1103/PhysRevLett.101.240404},
  issn =          {0031-9007},
  url =           {https://link.aps.org/doi/10.1103/PhysRevLett.101.240404},
}

@article{Lieb1994,
  author =        {Lieb, Elliott H.},
  journal =       {Phys. Rev. Lett.},
  month =         {oct},
  number =        {16},
  pages =         {2158--2161},
  title =         {{Flux Phase of the Half-Filled Band}},
  volume =        {73},
  year =          {1994},
  doi =           {10.1103/PhysRevLett.73.2158},
  issn =          {0031-9007},
  url =           {https://link.aps.org/doi/10.1103/PhysRevLett.73.2158},
}

@article{Kells2014,
  author =        {Kells, G. and Lahtinen, V. and Vala, J.},
  journal =       {Phys. Rev. B - Condens. Matter Mater. Phys.},
  number =        {7},
  pages =         {1--15},
  title =         {{Kitaev spin models from topological nanowire
                   networks}},
  volume =        {89},
  year =          {2014},
  abstract =      {We show that networks of superconducting topological
                   nanowires can realize the physics of exactly solvable
                   Kitaev spin models on trivalent lattices. This
                   connection arises from the low-energy theory of both
                   systems being described by a tight-binding model of
                   Majorana modes. In Kitaev spin models the Majorana
                   description provides a convenient representation to
                   solve the model, whereas in an array of Josephson
                   junctions of topological nanowires it arises from
                   localized physical Majorana modes tunneling between
                   the wire ends. We explicitly show that an array of
                   junctions of three wires—a setup relevant to
                   topological quantum computing with nanowires—can
                   realize the Yao-Kivelson model, a variant of Kitaev
                   spin models on a decorated honeycomb lattice.
                   Employing properties of the latter, we show that the
                   network can be constructed to give rise to
                   two-dimensional collective topological states
                   characterized by Chern numbers
  $\nu$=0,±1{\textless}math{\textgreater}{\textless}mrow{\textgreater}{\textless}mi{\textgreater}{\&}nu;{\textless}mo{\textgreater}={\textless}mn{\textgreater}0{\textless}mo{\textgreater},{\textless}mspace
  width="0.16em"{\textgreater}{\textless}mo{\textgreater}{\&}plusmn;{\textless}mn{\textgreater}1,
  and
  ±2{\textless}math{\textgreater}{\textless}mrow{\textgreater}{\textless}mo{\textgreater}{\&}plusmn;{\textless}mn{\textgreater}2,
  and that defects in the array can be associated with vortex-like
  quasiparticle excitations. In addition we show that the collective states are
  stable in the presence of disorder and superconducting phase fluctuations.
  When the network is operated as a quantum information processor, the
  connection to Kitaev spin models implies that decoherence mechanisms can in
  general be understood in terms of proliferation of the vortex-like
  quasiparticles.},
  doi =           {10.1103/PhysRevB.89.075122},
  issn =          {10980121},
}

@{Note1,
  key =           {Note1},
  note =          {enough to not have numerical issues},
}

@{Note2,
  key =           {Note2},
  note =          {Which in our case can be expressed as $C=\protect
                   \frac {1}{2\pi } \DOTSI \protect \MultiIntegral
                   {2}_{BZ}dq_x dq_y \protect \tmspace +\thinmuskip
                   {.1667em} \protect \frac {1}{2h_{\protect \textbf
                   {q}}^3}\left [\protect \frac {\partial }{\partial
                   _{q_x}}\protect \textbf {h}_{\protect \textbf {q}}(J)
                   \times \protect \frac {\partial }{\partial
                   _{q_y}}\protect \textbf {h}_{\protect \textbf {q}}(J)
                   \right ] \cdot \protect \textbf {h}_{\protect \textbf
                   {q}}(J)$.},
}

@{Note3,
  key =           {Note3},
  note =          {In general, the sign of this term coming from the
                   partial filling of the conduction band is always
                   opposite of that of the Chern number},
}

@{REVTEX41Control,
}

@{apsrev41Control,
  author =        {08},
  editor =        {1},
  pages =         {0},
  title =         {},
  year =          {1},
}


